The Complexity Landscape of Fixed-Parameter Directed Steiner Network Problems

Given a directed graph $G$ and a list $(s_1,t_1),\dots,(s_d,t_d)$ of terminal pairs, the Directed Steiner Network problem asks for a minimum-cost subgraph of $G$ that contains a directed $s_i\to t_i$ path for every $1\le i \le k$. The special case Directed Steiner Tree (when we ask for paths from a root $r$ to terminals $t_1,\dots,t_d$) is known to be fixed-parameter tractable parameterized by the number of terminals, while the special case Strongly Connected Steiner Subgraph (when we ask for a path from every $t_i$ to every other $t_j$) is known to be W[1]-hard. We systematically explore the complexity landscape of directed Steiner problems to fully understand which other special cases are FPT or W[1]-hard. Formally, if $\mathcal{H}$ is a class of directed graphs, then we look at the special case of Directed Steiner Network where the list $(s_1,t_1),\dots,(s_d,t_d)$ of requests form a directed graph that is a member of $\mathcal{H}$. Our main result is a complete characterization of the classes $\mathcal{H}$ resulting in fixed-parameter tractable special cases: we show that if every pattern in $\mathcal{H}$ has the combinatorial property of being "transitively equivalent to a bounded-length caterpillar with a bounded number of extra edges," then the problem is FPT, and it is W[1]-hard for every recursively enumerable $\mathcal{H}$ not having this property. This complete dichotomy unifies and generalizes the known results showing that Directed Steiner Tree is FPT [Dreyfus and Wagner, Networks 1971], $q$-Root Steiner Tree is FPT for constant $q$ [Such\'y, WG 2016], Strongly Connected Steiner Subgraph is W[1]-hard [Guo et al., SIAM J. Discrete Math. 2011], and Directed Steiner Network is solvable in polynomial-time for constant number of terminals [Feldman and Ruhl, SIAM J. Comput. 2006], and moreover reveals a large continent of tractable cases that were not known before.

==> preamble.tex <==
\usepackage{ifthen}
\usepackage{comment}
\makeatletter 
\pdfminorversion=5

\usepackage[
style=numeric-comp,
giveninits=true, 
maxbibnames=99, 
maxcitenames=2, 
natbib=true, 
labelnumber, 
backend=biber, 
sortcites=true,
doi=false,isbn=false,url=false
]{biblatex}
\let\oldcitet\citet
\renewcommand{\citet}[1]{\mbox{\oldcitet{#1}}}

\usepackage[margin=1in]{geometry}

\ifthenelse{\isundefined{\lipics}}
{
\usepackage[colorlinks=true,bookmarks=false]{hyperref}
\usepackage[small,bf]{caption}
\usepackage[pdftex]{graphicx}
\usepackage{subfigure}
\usepackage[british]{babel}
}
{}
\usepackage{xcolor}
\definecolor{darkblue}{rgb}{0,0,0.45}
\definecolor{darkred}{rgb}{0.6,0,0}
\definecolor{darkgreen}{rgb}{0.13,0.5,0}
\hypersetup{colorlinks, linkcolor=darkblue, citecolor=darkgreen, 
urlcolor=darkblue}

\ifthenelse{\isundefined{\llncs}}{
  \usepackage{amsthm}
  \usepackage{authblk}
  \renewcommand\Affilfont{\small}
}

\usepackage{amsmath,amsfonts,amssymb} 
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{wrapfig}
\usepackage{xspace}
\usepackage[shortlabels]{enumitem}
\setlist[enumerate]{nosep} %
\setlist[itemize]{nosep} %

%

\usepackage[raggedright]{titlesec}
\usepackage[ruled, linesnumbered, vlined]{algorithm2e}
\usepackage{csquotes}

\usepackage{aliascnt}
\ifthenelse{\isundefined{\llncs}}{
  \theoremstyle{plain} 
}{}
\newtheorem{thm}{Theorem}[section]
\newaliascnt{lem}{thm}
\newaliascnt{crl}{thm}
\newaliascnt{dfn}{thm}
\newaliascnt{claim}{thm}
\newaliascnt{prop}{thm}
\newcommand{\cqed}{\renewcommand{\qed}{\hfill$\lrcorner$}}
\newtheorem{lem}[lem]{Lemma} 
\newtheorem{claim}[claim]{Claim} 
\newtheorem{prop}[prop]{Proposition} 
\newtheorem{crl}[crl]{Corollary} 
\ifthenelse{\isundefined{\llncs}}{
  \theoremstyle{definition} 
}{}
\newtheorem{dfn}[dfn]{Definition}
\aliascntresetthe{lem}
\aliascntresetthe{crl}
\aliascntresetthe{prop}
\aliascntresetthe{dfn}
\aliascntresetthe{claim}
%
\providecommand*{\thmautorefname}{Theorem}
\providecommand*{\lemautorefname}{Lemma}
\providecommand*{\crlautorefname}{Corollary}
\providecommand*{\dfnautorefname}{Definition}
\providecommand*{\claimautorefname}{Claim}

%
\newcommand{\ol}[1]{{\overline{#1}}}
\newcommand{\mc}[1]{{\mathcal{#1}}}
\newcommand{\ms}[1]{\ensuremath{\mathscr{#1}}}
\newcommand{\eps}{{\varepsilon}}

\newcommand{\ignore}[1]{}
%

%
%
\usepackage{environ,xstring}
\newif\iflabel
\newif\ifdbs
\newif\ifamp
\NewEnviron{doitall}{%
  \noexpandarg
  \expandafter\IfSubStr\expandafter{\BODY}{\label}{\labeltrue}{\labelfalse}%
  \expandafter\IfSubStr\expandafter{\BODY}{\\}{\dbstrue}{\dbsfalse}%
  \expandafter\IfSubStr\expandafter{\BODY}{&}{\amptrue}{\ampfalse}%
  \iflabel\def\doitallstar{}\else\def\doitallstar{*}\fi
  \ifdbs
    \ifamp
      \def\doitallname{align}%
    \else
      \def\doitallname{multline}%
    \fi
  \else
    \def\doitallname{equation}
  \fi
  \begingroup\edef\x{\endgroup
    \noexpand\begin{\doitallname\doitallstar}%
    \noexpand\BODY
    \noexpand\end{\doitallname\doitallstar}%
  }\x
}
\def\[#1\]{\begin{doitall}#1\end{doitall}}

\makeatother 

\newcommand{\pname}[1]{\textsc{#1}}
%
%
%
%

